Seeing Eye to AI: Human Alignment via Gaze-Based Response Rewards for Large Language Models

Advancements in Natural Language Processing (NLP), have led to the emergence of Large Language Models (LLMs) such as GPT, Llama, Claude, and Gemini, which excel across a range of tasks but require extensive fine-tuning to align their outputs with human expectations. A widely used method for achieving this alignment is Reinforcement Learning from Human Feedback (RLHF), which, despite its success, faces challenges in accurately modelling human preferences. In this paper, we introduce GazeReward, a novel framework that integrates implicit feedback -- and specifically eye-tracking (ET) data -- into the Reward Model (RM). In addition, we explore how ET-based features can provide insights into user preferences. Through ablation studies we test our framework with different integration methods, LLMs, and ET generator models, demonstrating that our approach significantly improves the accuracy of the RM on established human preference datasets. This work advances the ongoing discussion on optimizing AI alignment with human values, exploring the potential of cognitive data for shaping future NLP research.

==> 11_summary.tex <==
To better understand the potential of cognitive data in improving machine learning models, specifically \textbf{\acrfull{llms}}, from TID, we propose \textbf{GazeReward} in our paper: \url{https://arxiv.org/pdf/2410.01532}. GazeReward is an innovative framework for aligning \acrshort{llms} with human preferences by incorporating \textbf{\acrfull{et}} data into reward modeling.

LLMs like GPT \citep{openai_gpt-4_2023}, Llama \citep{dubey_llama_2024}, and others have revolutionized \acrfull{nlp}, excelling in diverse tasks but often requiring fine-tuning to meet human expectations. A common approach to achieving human alignment involves leveraging explicit human feedback as \textbf{preference} information. Traditional approaches like \acrfull{rlhf} \citep{ouyang_training_2022} have been widely used, but they face challenges such as scalability, inconsistent human annotations, and high costs \citep{casper_open_2023}. Obtaining high-quality feedback from human annotators, usually provided after examining a model response, suffers from several caveats. For instance, low inter-annotator agreement can result in inconsistent evaluations of the same model output due to varying interpretations, domain expertise, or biases \citep{amodei_concrete_2016}.

Incorporating \acrshort{et} data into \acrshort{nlp} tasks has proven valuable, as demonstrated by numerous works \citep{huang_longer_2023, khurana_synthesizing_2023, hollenstein_advancing_2019, yang_plm-as_2023,kiegeland_pupil_2024, deng_pre-trained_2023, mathias_eyes_2018, mcguire_sentiment_2021}. Recently, \cite{kiegeland_pupil_2024} proposed the integration of \acrshort{et} in controlled sentiment generation to create a dataset that can be used in human alignment methods.

So, our work explores leveraging ET data, a form of implicit feedback that reflects cognitive and perceptual processes during reading and language comprehension, to better model preference modeling. The core idea of GazeReward is to use ET features to enhance the \textbf{\acrfull{rm}}, which is central to human alignment techniques. Eye-tracking captures oculomotor behavior—fixations, saccades, and reading patterns—that correlate with attention and information processing. Unlike explicit feedback, ET data is unbiased, temporally precise, and offers rich insights into user preferences \citep{zhang_eye-tracking_2024}. 

To integrate ET signals, we employed state-of-the-art \textbf{ET prediction models} to generate synthetic gaze features from text prompts and responses. These features were combined with text embeddings using two\textbf{methods}: GazeConcat, which concatenates embeddings, and GazeAdd, which adds them element-wise. We have conducted experiments using two \textbf{datasets}: OASST1 and HelpSteer2. These \textbf{datasets} include human-annotated preference pairs, where one response is preferred over another. The RM was fine-tuned using open-source LLMs such as Llama 3 and Mistral, with and without ET features. ET prediction models provided features like first fixation duration (FFD) and total reading time (TRT), which were integrated into the RM via a specially designed feature projector. Performance was measured by the RM’s \textbf{accuracy} in predicting human preferences, using both standard datasets and the RewardBench benchmark.

The \textbf{results} demonstrate that incorporating ET features significantly improves RM accuracy, with gains exceeding 20\% in some cases. While promising, our study has limitations. \textbf{Future work} could involve collecting task-specific ET data and extending the framework to other languages and larger models. Additionally, exploring alternative integration methods, such as modifying attention masks, could further enhance performance. GazeReward represents a significant step forward in aligning AI systems with human values by integrating cognitive data into reward modeling. This work not only improves the performance of existing models but also opens new avenues for research in \textbf{multimodal AI alignment}. By harnessing the power of gaze, we can make AI more aligned to human needs and expectations. \textbf{Check the paper for more details!}

